Fair Bayesian Optimization

Given the increasing importance of machine learning (ML) in our lives, several algorithmic fairness techniques have been proposed to mitigate biases in the outcomes of the ML models. However, most of these techniques are specialized to cater to a single family of ML models and a specific definition of fairness, limiting their adaptibility in practice. We introduce a general constrained Bayesian optimization (BO) framework to optimize the performance of any ML model while enforcing one or multiple fairness constraints. BO is a model-agnostic optimization method that has been successfully applied to automatically tune the hyperparameters of ML models. We apply BO with fairness constraints to a range of popular models, including random forests, gradient boosting, and neural networks, showing that we can obtain accurate and fair solutions by acting solely on the hyperparameters. We also show empirically that our approach is competitive with specialized techniques that enforce model-specific fairness constraints, and outperforms preprocessing methods that learn fair representations of the input data. Moreover, our method can be used in synergy with such specialized fairness techniques to tune their hyperparameters. Finally, we study the relationship between fairness and the hyperparameters selected by BO. We observe a correlation between regularization and unbiased models, explaining why acting on the hyperparameters leads to ML models that generalize well and are fair.

==> abstract.tex <==

\begin{abstract}
Given the increasing importance of machine learning (ML) in our lives, several algorithmic fairness techniques have been proposed to mitigate biases in the outcomes of the ML models. However, most of these techniques are specialized to cater to a single family of ML models and a specific definition of fairness, limiting their adaptibility in practice. We introduce a general constrained Bayesian optimization (BO) framework to optimize the performance of any ML model while enforcing one or multiple fairness constraints. BO is a model-agnostic optimization method that has been successfully applied to automatically tune the hyperparameters of ML models. We apply BO with fairness constraints to a range of popular models, including random forests, gradient boosting, and neural networks, showing that we can obtain accurate and fair solutions by acting solely on the hyperparameters. We also show empirically that our approach is competitive with specialized techniques that enforce model-specific fairness constraints, and outperforms preprocessing methods that learn fair representations of the input data. Moreover, our method can be used in synergy with such specialized fairness techniques to tune their hyperparameters. Finally, we study the relationship between fairness and the hyperparameters selected by BO. We observe a correlation between regularization and unbiased models, explaining why acting on the hyperparameters leads to ML models that generalize well and are fair.
\end{abstract}




==> background_bo.tex <==
\section{\Blackbox Bayesian Optimization}
\label{sec:background}
Bayesian optimization (BO) is a well-established methodology to optimize expensive opaque functions in a \blackbox manner~\citep[see][for an overview]{Shahriari2016}. It relies on a probabilistic model of the unknown target $f(\xb)$ one wishes to optimize and which is repeatedly queried until one runs out of budget (e.g., time). Queries consist in evaluations of $f$ at hyperparameter configurations $\xb^1,\ldots,\xb^n$ selected according to an explore-exploit trade-off criterion or \emph{acquisition function} \citep{Jones1998}. The hyperparameter configuration corresponding to the best query is then returned. One popular approach is to impose a Gaussian process (GP) prior over $f$ and, in light of the observed queries $f(\xb^1),\ldots,f(\xb^n)$, compute the posterior GP~\citep{Rasmussen2006}. The posterior GP is characterized by a posterior mean function and a posterior variance function that are required when evaluating the acquisition function for each new query of $f$. 

A widely used acquisition function is the Expected Improvement (EI) \citep{Mockus1978}. %
For a Gaussian predictive distribution, EI is defined in closed-form as the following: $EI(\xb)= \mathbf{E}[\max(0,f(\xb_{min})-f(\xb))] =\sigma^2(\xb)(z(\xb)\Phi_n(z(\xb))+\phi_n(z(\xb)))$, where $z(\xb) := \frac{\mu(\xb)-f(\xb_{min})}{\sigma^2(\xb)}$. $\mu$ and $\sigma^2$ are respectively the posterior GP mean and variance, and $\Phi_n$ and $\phi_n$ respectively the CDF and PDF of the standard normal. Alternative acquisition functions based on information gain criteria have been developed~\citep{Hennig2012}. Standard acquisitions only focus on the objective $f(\xb)$ and do not account for additional constraints. In this work, we aim to optimize an opaque function $f(\xb)$ subject to fairness constraints $c(\xb) \leq \epsilon$, $\epsilon \in \mathbb{R}$, with $\epsilon$ determining how strictly the fairness constraint should be enforced.



==> header.tex <==
\usepackage[utf8]{inputenc} %
\usepackage[T1]{fontenc}    %
\usepackage[hidelinks]{hyperref}       %
\usepackage{url}            %
\usepackage{booktabs}       %
\usepackage{amsfonts}       %
\usepackage{nicefrac}       %
\usepackage{microtype}      %
\usepackage{subfigure}
\usepackage{todonotes} %
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{adjustbox}
\usepackage{multirow}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{setspace}
\usepackage{accents}
\usepackage{epstopdf}
\usepackage{hyperref}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\R}{{\mathbb R}} 
\newcommand{\bbS}{{\mathbb S}} 
\newcommand{\E}{{\mathbb E}} 
\newcommand{\EI}{{\text{EI}}} 
\newcommand{\p}{{\mathbb P}} 
\newcommand{\N}{{\mathcal N}} 
\newcommand{\A}{{\mathbb A}} 
\newcommand{\I}{{\mathcal I}} 
\newcommand{\bigO}{{\mathcal O}} 
\newcommand{\LL}{{\mathcal L}} 

\DeclareMathOperator{\di}{d\!}
\DeclareMathOperator{\bx}{\mathbf{x}}
\DeclareMathOperator{\GP}{\mathcal{GP}}
\newcommand{\EIh}{\text{EI}h}
\newcommand{\bcdot}{{\boldsymbol{\cdot}}}
\newcommand{\by}{{\mathbf{y}}}
\newcommand{\bk}{{\mathbf{k}}}
\newcommand{\X}{{\mathcal{X}}}
\newcommand{\D}{{\mathcal{D}}}
\newcommand{\mI}{\mathsf{I}}
\newcommand{\mK}{\mathsf{K}}

==> nn_example.tex <==
\begin{figure*}
\centering
\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{input neuron}=[neuron, fill=green!50];
    \tikzstyle{output neuron}=[neuron, fill=red!50];
    \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
    \tikzstyle{black neuron}=[neuron, fill=black!80];
    \tikzstyle{annot} = [text width=4em, text centered]

    \foreach \name / \y in {1,...,4}
        \node[input neuron, pin=left:Input \#\y] (I-\name) at (0,-\y) {};

    \foreach \name / \y in {1,...,5}
        \path[yshift=0.5cm]
            node[hidden neuron] (H-\name) at (\layersep,-\y cm) {};

    \foreach \name / \y in {1,...,4}
            \node[input neuron] (Ho-\name) at (2*\layersep,-\y) {};

    \node[black neuron, right of=Ho-3] (B) at (2*\layersep,-2.5 cm) {};
    
    \node[output neuron,pin={[pin edge={->}]right:Output}, right of=B] (O) {};

    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,5}
            \path (I-\source) edge (H-\dest);

    \foreach \source in {1,...,5}
        \foreach \dest in {1,...,4}
            \path (H-\source) edge (Ho-\dest);

    \foreach \source in {1,...,4}
        \path (Ho-\source) edge (B);
        
    \path (B) edge (O);

    \node[annot,above of=H-1, node distance=1cm] (hl) {Hidden layer};
    \node[annot,right of=hl] (h2) {New representation};
    \node[annot,left of=hl] {Input layer};
    \node[annot,right of=h2] (bb) {Black-box};
    \node[annot,right of=bb] {Output layer};
    
    \draw[draw=black, line width=1mm] (1.4,-5.0) rectangle ++(7.3,6.5);
\end{tikzpicture}
\caption{The idea}
\label{fig:idea}
\end{figure*}
